A Parameter-Driven Physics-Informed Neural Network Framework for Solving Two-Parameter Singular Perturbation Problems Involving Boundary Layers

In this article, our goal is to solve two-parameter singular perturbation problems (SPPs) in one- and two-dimensions using an adapted Physics-Informed Neural Networks (PINNs) approach. Such problems are of major importance in engineering and sciences as it appears in control theory, fluid and gas dynamics, financial modelling and so on. Solutions of such problems exhibit boundary and/or interior layers, which make them difficult to handle. It has been validated in the literature that standard PINNs have low accuracy and can't handle such problems efficiently. Recently Cao et. al \cite{cao2023physics} proposed a new parameter asymptotic PINNs (PA-PINNs) to solve one-parameter singularly perturbed convection-dominated problems. It was observed that PA-PINNs works better than standard PINNs and gPINNs in terms of accuracy, convergence and stability. In this article, for the first time robustness of PA-PINNs will be validated for solving two-parameter SPPs.

==> strech.tex <==
\begin{lemma}\label{lemmaZt}
    Let $\mathfrak{u}^*$ and $\mathfrak{u}$ be  solutions of the sub-problems (\ref{ch2_x_full_dis}) and (\ref{ch5eq3.4}), respectively. Then we have the following estimate 
		\begin{align*}
& \left\{\begin{array}{l}
\left|\mathscr{Z}_t^*(\mathfrak{u}^{*},v_h^*)\right|  \leq C ( N^{-(k+1)}+\varepsilon^{1/2}(N^{-1}\ln N)^{(k+1)} )\Vert v_h^*\Vert_W^* , \\
\left|\mathscr{Z}_t(\mathfrak{u},v_h)\right| \leq C ( N^{-(k+1)}+\varepsilon^{1/2}(N^{-1}\ln N)^{(k+1)} )\Vert v_h\Vert_W .
\end{array}\right. \\
%& \forall n=0, \cdots, M-1 \text {, and } \forall i, j=0, \cdots, N .
\end{align*}
\end{lemma}
\begin{proof} We shall prove the first estimates since the second one follows similarly.
     We have from the solution decomposition that $\mathfrak{u}^*=v^*+w^*$. We recall the following interpolation error estimate from \cite{tobiska2006analysis}. For any $v^*\in H^{k+1}(I_{x_i})$ and its interpolation $\mathscr{I}_x v^*$, we have
    \begin{align} \label{tobiska} 
    |v^*-\mathscr{I}_x v^*|_{H^{l}(I_{x_i})}&\le C(h_i^{x})^{k+1-l}|v|_{H^{k+1}(I_{x_i})},\quad l=0,1,\ldots ,k+1. \end{align}
    By the Cauchy-Schwarz inequality 
    %It follows from Cauchy-Schwarz inequality that
    \begin{align*}
        \left|\mathscr{Z}_t^*(\mathfrak{u}^{*},v_h^*)\right| \leq \Vert\mathscr{I}_{x}\mathfrak{u}^*_t - \mathfrak{u}^*_t\Vert \Vert v_h^*\Vert_W^*.
    \end{align*}
    %Let  $\kappa^{*}:=v^*-\mathscr{I}_{x} v^*$. 
    From the interpolation error estimates (\ref{tobiska}), we get
 %   \begin{align}\label{eq-11}
 %       (\Vert \kappa^{*,n+1} \Vert_W^*)^2=( \vert \kappa^{*,n+1}\vert_1^*)^2+\Vert \sqrt{c_1} \kappa^{*,n+1}\Vert^2+(\vert \kappa^{*,n+1}\vert_C^*)^2=:T_1+T_2+T_3.
%    \end{align}
  %  Since $\kappa^{*,n+1}$ is continuous, we have $T_3=0$ and $s_d^*(\kappa^{*,n+1},\kappa^{*,n+1})=0$. It follows from $s_d^*(\kappa^{*,n+1},\kappa^{*,n+1})=0$,  (\ref{ch5eq2.7}), (\ref{ch5eq2.9}) and (\ref{tobiska}) that 
 %   \begin{align}
 %       \label{T_1}\begin{split}
%        T_1&\leq  \varepsilon \sum_{i=1}^N (h_{ i}^x)^{2k}\left\|v^*\left(t_{n+1}\right)\right\|_{H^{k+1}\left(I_{x_i}\right)}^2 \\
%& \leq C \varepsilon\left(\sum_{i=1}^{N / 2} (h_i^x)^{2k+1}+\sum_{i=N / 2}^N (h_i^x)^{2k+1}\right) \\
%& \leq C \varepsilon\left(1+(\varepsilon \ln N)^{2k+1}\right) N^{-2k} \\
%& \leq C N^{-2k}.\end{split}
%    \end{align}
   % Using the same idea, we can conclude that
     \begin{align}
        \label{T_2}\begin{split}
       \Vert\mathscr{I}_{x}v^*_t - v^*_t\Vert &\leq   \sum_{i=1}^N (h_{ i}^x)^{2(k+1)}\left\|v^*_t\right\|_{H^{k+1}\left(I_{x_i}\right)}^2 \\
& \leq C N^{-2(k+1)}.\end{split}
\end{align}
For the layer component $w^*$, let $\kappa^*:=w^*- \mathscr{I}_{x} w^*$. We then compute 
\begin{align}\label{T_1}
    \begin{split}
        \begin{aligned}
 \left\|\kappa_t^*\right\|_{L^2\left(\Omega_x\right)}^2 
 &=\left\|\kappa_t^*\right\|_{L^2\left(\left[0,1-\sigma_z\right]\right)}^2+ 
\sum_{i=N / 2+1}^N\left\|\kappa_t^*\right\|_{L^2\left(I_{x_i}\right)}^2 \\
& \leq C\left(1-\sigma_x\right)\left\|\kappa_t^*\right\|_{L^{\infty}\left(\left[0,1-\sigma_x\right]\right)}^2+ \\
& C \sum_{i=N / 2+1}^N h_{x_ i}^{2(k+1)} \int_{x_{i-1}}^{x_i}\left|( w^*_t)_x^{(k+1)}\right|^2 d x \\
& \leq C\left\{\left\|w^*_t\right\|_{L^{\infty}\left(\left[0,1-\sigma_z\right]\right)}^2+\sum_{i=N / 2+1}^N h_{x_ i}^{2(k+1)} \int_{x_{i-1}}^{x_i} \varepsilon^{-2(k+1)} e^{\frac{-2 \beta_x(1-x)}{\epsilon}} d x\right\} \\
& \leq C\left\{\max _{\left[0,1-\sigma_x\right]}\left\{e^{\frac{-2 \beta_x(1-z)}{\epsilon}}\right\}+\varepsilon (N^{-1}\ln N)^{2(k+1)}\right\} \\
& \leq C ( N^{-2(k+1)}+\varepsilon(N^{-1}\ln N)^{2(k+1)} ).
\end{aligned}
    \end{split}
\end{align}



From (\ref{T_1}) and (\ref{T_2}), we reach the conclusion. Thus, we complete the proof.



\end{proof}
\begin{proof}
    \begin{align*}
        \left(\eta_{0,j}^{*,n+1}, \phi\right) + A^{*}\left(\eta_{h,j}^{*,n+1}, \phi\right) &= \left(\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right) + A^{*}\left(\mathfrak{u}_{h}^{*,n+1}, \phi\right) 
        - \left(R_{0,h}\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right) - A^{*}\left(R_{h}\mathfrak{u}{*,n+1}, \phi\right) \\
        &= \left(\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right) + A^{*}\left(\mathfrak{u}{h}^{*,n+1}, \phi\right) + \left(\mathscr{I}_{0,h}\Hat{u}_{0,h,j}^{*, n+1} - R_{0,h}\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right)\\
        & \quad - \left(\mathscr{I}_{0,h}\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right) - A^{*}\left(R_{h}\mathfrak{u}{*,n+1}, \phi\right) \\
        & = \left(\Hat{\zeta}_{0,h,j}^{*,n+1}, \phi_{0}\right) - \left(\mathscr{L}_{x}\mathfrak{u}{*,n+1}, \phi\right) +\left(f_{1}^{n+1}, \phi_{0}\right) -  \left(\mathscr{I}_{0,h}\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right)\\
         & = \left(\Hat{\zeta}_{0,h,j}^{*,n+1}, \phi_{0}\right) - \left(\mathscr{I}_{0,h}\mathscr{L}_{x}\mathfrak{u}{*,n+1}, \phi\right) + \left(\mathscr{I}_{0,h}f_{1}^{n+1}, \phi_{0}\right) -  \left(\mathscr{I}_{0,h}\Hat{u}_{0,h,j}^{*, n+1}, \phi_{0}\right)\\
         & = \left(\Hat{\zeta}_{0,h,j}^{*,n+1}, \phi_{0}\right) - \left(\mathscr{I}_{0,h}(\psi^{n+1}), \phi_{0}\right).
    \end{align*}
    
\end{proof}
